Application of Deep Learning Methods in Monitoring and Optimization of Electric Power Systems

This PhD thesis thoroughly examines the utilization of deep learning techniques as a means to advance the algorithms employed in the monitoring and optimization of electric power systems. The first major contribution of this thesis involves the application of graph neural networks to enhance power system state estimation. The second key aspect of this thesis focuses on utilizing reinforcement learning for dynamic distribution network reconfiguration. The effectiveness of the proposed methods is affirmed through extensive experimentation and simulations.

==> chapter_02/state_estimation.tex <==
\chapter{Power System State Estimation}	\label{ch:se_power}
\addcontentsline{lof}{chapter}{2 Power System State Estimation}
In this chapter, we review the state-of-the-art SE models in electric power systems. The power system represents a dynamic system, where power generation and power demand is changing values depending on various factors. The SE is used for describing the present state of the power system, unlike the power flow analysis which is used for defining load profiles, generator capabilities, voltage specification, contingency analysis, and planning. 
	\begin{figure}[ht]
	\centering
	\includegraphics[width=9.5cm]{./chapter_02/Figs/fig1_1.eps}
	\caption{EMS configuration and SE routines.}
	\label{fig1_1}
	\end{figure}

The SE is a part of the energy management systems (EMS) and typically includes network topology processors, observability analysis, SE algorithm and bad data analysis, as shown in \autoref{fig1_1}. Data for the SE arrives from SCADA and WAMS technology. SCADA provides legacy measurements with low sampling rates insufficient to capture system dynamics in real-time and provides a snapshot SE with order of seconds and minutes latency. In contrast, WAMS provides data from PMUs with high sampling rates $(10\,\mbox{ms} - 20\,\mbox{ms})$ enabling the real-time system monitoring.

In a usual scenario, the SE model is described with the system of non-linear equations, where bus voltage magnitudes and bus voltage angles, transformer magnitudes of turns ratio and transformer angles of turns ratio as state variables $\mathbf{x}$. The core of the SE is the SE algorithm that provides an estimate of the system state $\mathbf{x}$ based on the network topology and available measurements. SE is performed on a bus/branch model and used to reconstruct the state of the system. Conventional SE algorithms are centralized and typically use the Gauss-Newton method to solve the non-linear WLS problem \cite{monticelli, schweppe}. Besides the non-linear SE model, the DC model is obtained by linearization of the non-linear model, and it provides an approximate solution. The DC state estimate is obtained through non-iterative procedure by solving the linear WLS problem.


\section{Measurement Model}	\label{sec:Measurement_Model}
The SE algorithm estimates the values of the state variables based on the knowledge of network topology and parameters, and measured values obtained from measurement devices spread across the power system. The knowledge of the network topology and parameters is provided by the network topology processor in the form of the bus/branch model, where branches of the grid are usually described using the two-port $\pi$-model \cite[Ch.~1,2]{abur}. The bus/branch model can be represented using a graph $\mathcal{G} =$ $(\mathcal{H},\mathcal{E})$, where the set of nodes $\mathcal{H} =$ $\{1,\dots,N  \}$ represents the set of buses, while the set of edges $\mathcal{E} \subseteq \mathcal{H} \times \mathcal{H}$ represents the set of branches of the power network. 

As an input, the SE requires a set of measurements $\mathcal{M}$ of different electrical quantities spread across the power network. Using the bus/branch model and available measurements, the observability analysis defines observable and unobservable parts of the network, subsequently defining the additional set of pseudo-measurements needed to determine the solution \cite[Ch.~4]{abur}.
Finally, the measurement model can be described as the system of equations \cite{schweppe}:  
		\begin{equation}
        \begin{aligned}
        \mathbf{z}=\mathbf{h}(\mathbf{x})+\mathbf{u},
        \end{aligned}
		\label{SE_model}
		\end{equation}
where $\mathbf {x}=[x_1,\dots,x_{n}]^{\mathrm{T}}$ is the vector of the state variables, $\mathbf{h}(\mathbf{x})=$ $[h_1(\mathbf{x})$, $\dots$, $h_k(\mathbf{x})]^{\mathrm{T}}$ is the vector of measurement functions,  $\mathbf{z} = [z_1,\dots,z_k]^{\mathrm{T}}$ is the vector of measurement values, and $\mathbf{u} = [u_1,\dots,u_k]^{\mathrm{T}}$ is the vector of uncorrelated measurement errors. The SE problem in transmission grids is commonly an overdetermined system of equations $(k>n)$ \cite[Sec.~2.1]{monticelliBook}.

Each measurement $M_i \in \mathcal{M}$ is associated with measured value $z_i$, measurement error  $u_i$, and measurement function $h_i(\mathbf{x})$. Under the assumption that measurement errors $u_i$ follow a zero-mean Gaussian distribution, the probability density function associated with the \textit{i}-th measurement is proportional to:
		\begin{equation}
        \begin{gathered}
        \mathcal{N}(z_i|\mathbf{x},v_i) \propto
        \exp\Bigg\{\cfrac{[z_i-h_i(\mathbf{x})]^2}{2v_i}\Bigg\},
        \end{gathered}
		\label{SE_Gauss_mth}
		\end{equation}
where $v_i$ is the measurement variance defined by the measurement error  $u_i$, and the measurement function $h_i(\mathbf{x})$ connects the vector of state variables $\mathbf{x}$ to the value of the \textit{i}-th measurement.

The SE in electric power systems deals with the problem of determining state variables $\mathbf{x}$ according to the noisy observed data $\mathbf{z}$ and a prior knowledge: 
		\begin{equation}
        \begin{gathered}
 		p(\mathbf{x}|\mathbf{z})=
		\cfrac{p(\mathbf{z}|\mathbf{x})p(\mathbf{x})}{p(\mathbf{z})}.
        \end{gathered}
		\label{SE_problem}
		\end{equation}
Assuming that the prior probability distribution $p(\mathbf{x})$ is uniform, and given that $p(\mathbf{z})$ does not depend on $\mathbf{x}$, the maximum a posteriori (MAP) solution of \eqref{SE_problem} reduces to the maximum likelihood solution, as given below \cite{barber}:
		\begin{equation}
        \begin{gathered}
		\hat{\mathbf{x}}=
		\mathrm{arg}\max_{\mathbf{x}}p(\mathbf{x}|\mathbf{z})=
		\mathrm{arg}\max_{\mathbf{x}}p(\mathbf{z}|\mathbf{x})=
		\mathrm{arg}\max_{\mathbf{x}}\mathcal{L}(\mathbf{z}|\mathbf{x}).
        \end{gathered}
		\label{SE_MAP_MLE}
		\end{equation}

\begin{tcolorbox}[title=Maximum Likelihood Estimator]
One can find the solution \eqref{SE_MAP_MLE} via maximization of the likelihood function $\mathcal{L}(\mathbf{z}|\mathbf{x})$, which is defined via likelihoods of $k$ independent measurements:  
		\begin{equation}
        \begin{gathered}
		\hat{\mathbf x}=
		\mathrm{arg} \max_{\mathbf{x}}\mathcal{L}(\mathbf{z}|\mathbf{x})=
		\mathrm{arg} \max_{\mathbf{x}}  
		\prod_{i=1}^k \mathcal{N}(z_i|\mathbf{x},v_i).
        \end{gathered}
		\label{SE_likelihood}
		\end{equation}
\end{tcolorbox}

It can be shown that the solution of the MAP problem can be obtained by solving the following optimization problem, known as the WLS problem \cite[Sec.~9.3]{wood}:
		\begin{equation}
        \begin{gathered}
		\hat{\mathbf x} =
		\mathrm{arg}\min_{\mathbf{x}} \sum_{i=1}^k 
		\cfrac{[z_i-h_i(\mathbf x)]^2}{v_i}.
        \end{gathered}
		\label{SE_WLS_problem}
		\end{equation}
The state estimate $\hat{\mathbf x}$ representing the solution of the optimization problem \eqref{SE_WLS_problem} is known as the WLS estimator, the maximum likelihood and WLS estimator are equivalent to the maximum a posteriori (MAP) solution \cite[Sec.~8.6]{barber}.



\subsection{Measurement Set}
The typical set of measurements $\mathcal{M}$ is defined according to type of measurement devices and includes:

\begin{enumerate}[label=(\roman*)]
\item Legacy measurements that contain active and reactive power flow and line current magnitude $\{M_{P_{ij}},$ $M_{Q_{ij}},$ $M_{I_{ij}} \}$, $(i,j) \in \mathcal{E}$, respectively; active and reactive power injection and bus voltage magnitude $\{M_{P_{i}},$ $M_{Q_{i}},M_{V_{i}} \}$, $i \in \mathcal{H}$, respectively.
\item Phasor measurements provide by PMUs contain line current $\mathcal{M}_{\ph{I}_{ij}}$, $(i,j) \in \mathcal{E}$ and bus voltage $\mathcal{M}_{\ph{V}_{i}}$, $i \in \mathcal{H}$ phasors, where each phasor measurement can be represented by a pair of measurements, for example, the bus voltage phasor measurement can be represented over the bus voltage magnitude and angle measurements $\mathcal{M}_{\ph{V}_{i}} =$ $\{{M}_{{V}_{i}}, {M}_{{\theta}_{i}}\}$, $i \in \mathcal{H}$.
\end{enumerate}

Each legacy measurement is described by non-linear measurement function $h_i(\mathbf{x})$, where the state vector $\mathbf{x}$ is given in polar coordinates. In contrast, phasor measurements can be described with both non-linear and linear measurement functions $h_i(\mathbf{x})$, where the state vector $\mathbf{x}$ can be given in polar or rectangular coordinates. Phasor measurements integration into the SE defines different models for solving the SE problem. 


\subsection{The Equivalent Branch Model} \label{subsec:pi_model}
To solve SE problem, it is necessary to establish expressions of measurement functions  $\mathbf h (\mathbf x)$ related to measurements in the set $\mathcal{M}$. The equivalent $\pi$-model for a branch, shown in \autoref{fig1_2}, is sufficient to describe all measurement functions using currents, voltages and apparent powers. For simplicity, we assume that the model does not contain phase-shifting transformers.

The series admittance is $y_{ij}$ and shunt admittances of the branch are denoted as $y_{\mathrm{s}i} =$ $g_{\mathrm{s}i} + $ $\mathrm{j} b_{\mathrm{s}i}$ and $y_{\mathrm{s}j} =$ $g_{\mathrm{s}j} + $ $\mathrm{j} b_{\mathrm{s}j}$.
	\begin{figure}[ht]
	\centering
	\includegraphics[width=65mm]{./chapter_02/Figs/fig1_2.eps}
	\caption{The equivalent branch $\pi$-model.
	\label{fig1_2}}
	\end{figure}
The branch series admittance $y_{ij}$ is inversely proportional to the branch series impedance $z_{ij}$:  
	\begin{equation}
   	\begin{aligned}
    y_{ij} = \frac{1}{z_{ij}} = 
    \frac{1}{{r_{ij}}+\mathrm{j}x_{ij}} = 
    \frac{r_{ij}}{r_{ij}^2+x_{ij}^2}-
    \mathrm{j}\frac{x_{ij}}{r_{ij}^2+x_{ij}^2}=g_{ij}+\mathrm{j}b_{ij},
   	\end{aligned}
   	\label{br_admittance}
	\end{equation}
where $r_{ij}$ is a resistance, $x_{ij}$ is a reactance, $g_{ij}$ is a conductance and $b_{ij}$ is a susceptance of the branch. In \autoref{fig1_2}, $\{i,j\} \in \mathcal{H}$ denotes buses, where, in power networks the bus represents elements such as a generator, load, substation, etc.

Using Kirchoff's laws, the complex current at buses $i$ and $j$ are:
	\begin{subequations}
   	\begin{align}
    \ph{I}_{ij} &= 
    {y}_{ij}(\ph{V}_{i}-\ph{V}_{j})+{y}_{\mathrm{s}i}
    \ph{V}_{i}=
    ({y}_{ij}+{y}_{\mathrm{s}i})\ph{V}_{i}-{y}_{ij}\ph{V}_{j}
    \label{current_ij}\\
    \ph{I}_{ji} &=
    - {y}_{ij}(\ph{V}_{i}-\ph{V}_{j})+{y}_{\mathrm{s}j}
    \ph{V}_{j}=
    ({y}_{ij}+{y}_{\mathrm{s}j})\ph{V}_{j}-{y}_{ij}\ph{V}_{i}.
    \label{current_ji}
   	\end{align}
   	\label{current_ij_ji}%
	\end{subequations}		
From \eqref{current_ij_ji} the complex currents at the bus are proportional to admittances incident to the bus (i.e. the sum of admittances) and the admittance between buses. These equations refer to the Node-Voltage method, and we apply \eqref{current_ij} to derive SE models (i.e., measurement functions). Further, complex bus voltages can be written:
	\begin{subequations}
   	\begin{align}
    \ph{V}_{i}&=V_{i}\mathrm{e}^{\mathrm{j}\theta_{i}} 
    = V_i\cos\theta_i + \mathrm{j}V_i\sin\theta_i \label{vol_polar1} \\ 
    \ph{V}_{j}&=V_{j}\mathrm{e}^{\mathrm{j}\theta_{j}}  
    = V_j\cos\theta_j + \mathrm{j}V_j\sin\theta_j, 
   	\end{align}
   	\label{vol_polar}%
	\end{subequations}
where $V_i$ and $V_j$ are bus voltage magnitudes, and $\theta_i$ and $\theta_j$ are bus voltage angles at buses $i$ and $j$. The apparent power $\ph S_{ij}$ from bus $i$ to bus $j$ is equal to:
	\begin{equation}
   	\begin{aligned}
	\ph {S}_{ij}&=\ph{V}_i \ph{I}_{ij}^* = P_{ij}+\mathrm{j}Q_{ij},
	\end{aligned}
   	\label{apparent_ij}
	\end{equation}
where $P_{ij}$ and $Q_{ij}$ represent active and reactive power flow from bus $i$ to bus $j$. 

Further, the injection complex current into the bus $i \in \mathcal{H}$ can be obtained by observing a set of buses $\mathcal{H}_i \setminus i = \{k, \dots, K\} \subset \mathcal{H}$ connected to the bus $i$, illustrated in \autoref{fig1_3}. 
	\begin{figure}[ht]
	\centering
	\includegraphics[width=48mm]{./chapter_02/Figs/fig1_3.eps}
	\caption{The set of buses $\mathcal{H}_i \setminus i = \{k, \dots, K\} 
	\subset \mathcal{H}$ connected to the bus $i$.} 
	\label{fig1_3}
	\end{figure}	
Using Kirchoff's law and \eqref{current_ij}, the injection complex current $\ph{I}_{i}$ into the bus $i$ is defined:
	\begin{equation}
   	\begin{aligned}
    \ph{I}_{i} = 
    \ph{I}_{ik}+...+\ph{I}_{iK}= 
    \sum\limits_{j \in \mathcal{H}_i \setminus i} 
    \Big[({y}_{ij}+{y}_{\mathrm{s} i})
    \ph{V}_{i}-{y}_{ij}\ph{V}_{j} \Big].  
   	\end{aligned}
   	\label{injcurr_sum}
	\end{equation}

In general, for the electric power system with $\mathcal{H} =$ $\{1,\dots,N  \}$ buses, the injection complex current $\ph{I}_{i}$ for each bus $i \in \mathcal{H}$ can be computed using:
	\begin{equation}
   	\begin{aligned}
    \ph{I}_{i} =\sum\limits_{j=1}^N \Big[({y}_{ij}+{y}_{\mathrm{s}i})
    \ph{V}_{i}-{y}_{ij}\ph{V}_{j} \Big].
   	\end{aligned}
   	\label{injcurr_vol_all}
	\end{equation}
Further, the expanded form is:
	\begin{equation}
   	\begin{aligned}
    Y_{11}&\ph{V}_{1}+Y_{12}\ph{V}_{2}+Y_{13}\ph{V}_{3} + 
    \cdots+ Y_{1N}\ph{V}_{N}= \ph{I}_{1} \\
    Y_{21}&\ph{V}_{1}+Y_{22}\ph{V}_{2}+Y_{23}\ph{V}_{3} + 
    \cdots+ Y_{2N}\ph{V}_{N}= \ph{I}_{2} \\
    \;\vdots  & \\
    Y_{N1}&\ph{V}_{1}+Y_{N2}\ph{V}_{2}+Y_{N3}\ph{V}_{3} + 
    \cdots+ Y_{NN}\ph{V}_{N}= \ph{I}_{N}.
   	\end{aligned}
   	\label{injcurr_expa}
	\end{equation}
Above system of equations can be written in the the matrix form:
	\begin{equation}
   	\begin{aligned}
    \mathbf{Y}\pmb{\mathscr{V}}=\pmb{\mathscr{I}},
   	\end{aligned}
   	\label{injcurr_mat}
	\end{equation}
where the elements of the bus or nodal admittance matrix $\mathbf{Y}$, when the bus is incident to the branch, can be formed as:
	\begin{equation}
   	\begin{aligned}
  	Y_{ij}= G_{ij} + \mathrm{j}B_{ij} = 
  	\begin{cases}
   	\sum\limits_{j\in \mathcal{H}_i \setminus i} 
   	({y}_{ij}+{y}_{\mathrm{s}i}), & \text{if} \;\; i=j 
   	 \;\;(\mathrm{diagonal\;element})\\
   	-{y}_{ij}, & \text{if} \;\; i \not = j
   	 \;\;(\mathrm{non-diagonal\;element).}
	\end{cases}
	\end{aligned}
   	\label{adm_mat_ele}
	\end{equation}
When the branch is not incident (or adjacent) to the bus the corresponding element in the nodal admittance matrix $\textbf{Y}$ is equal to zero. The nodal admittance matrix $\mathbf{Y}$ is a sparse matrix (i.e., a small number of elements are non-zeros) for a real power systems. Note that, if bus $i$ contains shunt element (capacitor or reactor), positive or negative susceptance value will be added to the diagonal element $i = j$ of the matrix $\mathbf{Y}$. Although it is often assumed that the matrix $\mathbf{Y}$ is symmetrical, it is not a general case, for example, in the presence of phase shifting transformers the matrix $\mathbf{Y}$ is not symmetrical \cite[Sec.~9.6]{stevenson}.

The apparent power injection $\ph S_i$ into the bus $i$ is a function of the complex voltage $\ph{V}_i$ at the bus and the conjugate value of the injection complex current $\ph{I}_i$ into the bus $i$:
	\begin{equation}
   	\begin{aligned}
  	\ph {S}_{i} =\ph{V}_{i}\ph{I}_{i}^* = P_i + \mathrm{j}Q_i,
	\end{aligned}
   	\label{apparent_inj}
	\end{equation}
where $P_i$ and $Q_i$ represent active power and reactive power injection into bus $i$. According to \eqref{injcurr_expa}, \eqref{adm_mat_ele} and \eqref{apparent_inj} apparent injection power $S_i$ into the bus $i$ is:
	\begin{equation}
   	\begin{aligned}
   	\ph {S}_{i} =\ph{V}_{i}\sum\limits_{j \in \mathcal{H}_i} {Y}_{ij}^*
   	\ph{V}_{j}^*,                   
	\end{aligned}
   	\label{apparent_inj_vol}
	\end{equation}
where $\mathcal{H}_i$ is the set of buses adjacent to the bus $i$, including the bus $i$. Using \eqref{vol_polar}, apparent injection power $\ph S_i$ is defined:
	\begin{equation}
   	\begin{aligned}
   	\ph {S}_{i} ={V}_{i}\sum\limits_{j \in \mathcal{H}_i} {V}_{j}
   	\mathrm{e}^{\mathrm{j}\theta_{ij}}(G_{ij}-\mathrm{j}B_{ij}).   
	\end{aligned}
   	\label{apparent_inj_state}
	\end{equation}


\subsection{State Variables}
In typical scenario, the SE model takes complex bus voltages and transformer turns ratio as state variables $\mathbf{x}$. Without loss of generality, in the rest of the thesis, for the SE model we observe complex bus voltages $\ph V_i$, $i \in \mathcal{H}$ as state variables: 
	\begin{equation}
   	\begin{aligned}
    \ph V_i = V_{i}\mathrm{e}^{\mathrm{j}\theta_{i}} = 
    \Re {(\ph V_i)} + \mathrm{j} \Im{(\ph V_i)},
   	\end{aligned}
   	\label{state_vol}
	\end{equation} 
where $\Re {(\ph V_i)}$ and $\Im{(\ph V_i)}$ represent the real and imaginary components of the complex bus voltage $\ph V_i$, respectively.   

Thus, the vector of state variables $\mathbf{x}$ can be given in polar coordinates $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, where we observe bus voltage angles and magnitudes as state variables respectively: 
	\begin{equation}
   	\begin{aligned}
    \bm \uptheta&=[\theta_1,\dots,\theta_N]\\
    \mathbf V&=[V_1,\dots, V_N].
   	\end{aligned}
   	\label{polar_coord}
	\end{equation} 
One voltage angle from the vector $\bm \uptheta$ corresponds to the slack or reference bus where the voltage angle has a given value. Consequently, the SE operates with  $n=2N - 1$ state variables\footnote{For convenience, BP-based SE algorithms take state variables defined with \eqref{polar_coord} as probabilistic variable nodes, where each state variable defines a variable node (i.e., the number of state variables is $n=2N$).}. The conventional SE model in the presence of legacy measurements usually implies above approach. 

Furthermore, the vector of state variables $\mathbf{x}$ can be given in rectangular coordinates $\mathbf x \equiv[\mathbf{V}_\mathrm{re},\mathbf{V}_\mathrm{im}]^{\mathrm{T}}$, where we can observe real and imaginary components of bus voltages as state variables:   
	\begin{equation}
   	\begin{aligned}
    \mathbf{V}_\mathrm{re}&=\big[\Re(\ph{V}_1),\dots,\Re(\ph{V}_N)\big]\\
	\mathbf{V}_\mathrm{im}&=\big[\Im(\ph{V}_1),\dots,\Im(\ph{V}_N)\big].     
   	\end{aligned}
   	\label{rect_coord}
	\end{equation} 
One of the elements from the vector $\mathbf{V}_\mathrm{im}$ corresponds to the slack bus. This way of assignment is frequently used for phasor measurements, whereupon measurement functions $h_i(\mathbf{x})$ become linear. However, same as before, the number of state variables is $n=2N - 1$. 


\section{State Estimation Models} \label{subsec:se_models}
Power system SE models can be defined in several ways by using different criteria, such as type of measurements or according to state variables and measurements representation, as well as whether the system is linear or non-linear and how to interpret the obtained state estimator. 

\autoref{fig1_4} shows SE models described with measurement functions that precisely follow the physical laws. In general, the model where only legacy measurements exist is described with non-linear measurement functions, where state variables are given in the polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, and it defines the conventional SE model, described in \autoref{sub:leg_meas}.
    \begin{figure}[ht]
    \centering
    \includegraphics[width=11.5cm]{./chapter_02/Figs/fig1_4.eps}
    \caption{SE models described with measurement functions 
    that precisely follow the physical laws.}
    \label{fig1_4}
    \end{figure}

The simultaneous SE model represents the expansion of the conventional SE model with phasor measurements. State variables are given in the polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, while phasor measurements can be given in the polar or rectangular coordinates. Phasor measurements in polar coordinate system enable straightforward inclusion in the conventional SE model (see \autoref{sub:pmu_polar}), whereas it is necessary to convert measurement variances for the case of phasor measurements in the rectangular coordinate system (see \autoref{sub:pmu_rect}) \cite{catalina}.

Hybrid SE models \cite{yang, kashyap, ghosh, dzafic, phadke} use advantages of linear functions related to phasor measurements, where state variables are given in the rectangular coordinate system $\mathbf x \equiv[\mathbf{V}_\mathrm{re},\mathbf{V}_\mathrm{im}]^{\mathrm{T}}$. Finally, to provide a state estimator only with PMUs, the system needs to be observable by PMUs only, which is currently difficult to achieve. However, with the evolution and adoption of PMU technology and, consequently, decline in the price of PMUs, it is realistic to assume that future power systems will be fully observable by PMUs, where the SE model becomes linear \cite{gol}, as will be described in \autoref{sub:pmu_linear}.

\autoref{fig1_5} shows SE models related to the SE accuracy and solving methods. In the presence of legacy measurements where measurement functions follow the physical laws, the SE model represents the non-convex problem and the Gauss-Newon provides a solution, described in \autoref{subsec:gauss-newton}.  
    \begin{figure}[ht]
    \centering
    \includegraphics[width=5.9cm]{./chapter_02/Figs/fig1_5.eps}
    \caption{Different SE models related to the SE accuracy and solving methods.}
    \label{fig1_5}
    \end{figure}

The approximate solution is related with the DC SE model, obtained by linearisation of the non-linear model. The DC model ignores the reactive powers and transmission losses and takes into account only the active powers. Therefore, the DC SE takes only bus voltage angles as state variables, see \autoref{sec:dc_se_model}.     
 
Electric power systems observable by PMUs results with linear SE model where measurement functions follow the physical laws, thus obtained solution represent the optimal or exact state estimator. This model is beyond the thesis scope.  

\section{The Gauss-Newton Method} \label{subsec:gauss-newton}
In the presence of both, legacy and phasor measurements, the system \eqref{SE_model} in general represents the system of non-linear equations. The Gauss-Newton method is typically used to solve the non-linear SE model defined using measurement functions $\mathbf {h(x)}$ that precisely follow the physical laws that connect the measured variables and the state variables.  

\begin{tcolorbox}[title=Gauss-Newton Method]
Based on the available set of measurements $\mathcal{M}$, the WLS estimator $\hat{\mathbf x}$, i.e., the solution of the WLS problem \eqref{SE_WLS_problem}, can be found using the Gauss-Newton method:	
		\begin{subequations}
        \begin{gather}  
		\Big[\mathbf J (\mathbf x^{(\nu)})^\mathrm{T} \mathbf R^{-1} 
		\mathbf J (\mathbf x^{(\nu)})\Big] \Delta \mathbf x^{(\nu)} =
		\mathbf J (\mathbf x^{(\nu)})^\mathrm{T}
		\mathbf R^{-1} \mathbf r (\mathbf x^{(\nu)})
		\label{AC_GN_increment}\\
		\mathbf x^{(\nu+1)} = 
		\mathbf x^{(\nu)} + \Delta \mathbf x^{(\nu)}, \label{AC_GN_update}
        \end{gather}
        \label{AC_GN}%
		\end{subequations}	
where $\nu = \{0,1,2,\dots\}$ is the iteration index, $\Delta \mathbf x \in \mathbb {R}^{n}$ is the vector of increments of the state variables, $\mathbf J (\mathbf x)\in \mathbb {R}^{k\mathrm{x}n}$ is the Jacobian matrix of measurement functions $\mathbf h (\mathbf x)$ at $\mathbf x=\mathbf x^{(\nu)}$, $\mathbf{R}\in \mathbb {R}^{k\mathrm{x}k}$ is a measurement error covariance matrix, and $\mathbf r (\mathbf x) = \mathbf{z} - \mathbf h (\mathbf x)$ is the vector of residuals \cite[Ch.~10]{monticelliBook}. Note that, assumption that measurement errors are uncorrelated leads to the diagonal covariance matrix $\mathbf {R}$ that corresponds to measurement variances.
\end{tcolorbox}	

The non-linear SE represents non-convex problem arising from the non-linear measurement functions \cite{weng}. Due the fact that the values of state variables usually fluctuate in narrow boundaries, the non-linear SE model represents the mildly non-linear problem, where solutions are in a reasonable-sized neighborhood which enables the use of the Gauss-Newton method. The Gauss-Newton method can produce different rates of convergence, which can be anywhere from linear to quadratic \cite[Sec.~9.2]{hansen}. The convergence rate in regards to power system SE depends of the topology and measurements, and if parameters are consistent (e.g., free bad data measurement set), the method shows near quadratic convergence rate \cite[Sec.~11.2]{monticelliBook}.


\section{Legacy Measurments} \label{sub:leg_meas}
In the following, we provide expressions for measurement functions $\mathbf h (\mathbf x)$ and corresponding Jacobian elements of the matrix $\mathbf J (\mathbf x)$ related to legacy measurements, where state variables (i.e., unknown variables) are given in polar coordinates $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$. To recall, legacy measurements contain active and reactive power flow and line current magnitude $\{M_{P_{ij}},$ $M_{Q_{ij}},$ $M_{I_{ij}}\}$, $(i,j) \in \mathcal{E}$, respectively; active and reactive power injection and bus voltage magnitude $\{M_{P_{i}},$ $M_{Q_{i}},M_{V_{i}} \}$, $i \in \mathcal{H}$, respectively.  

The active and reactive power flow at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ can be obtained using \eqref{current_ij}, \eqref{vol_polar} and \eqref{apparent_ij}. It is easy to show that the apparent power $\ph S_{ij}$ equals:
	\begin{equation}
   	\begin{aligned}
	\ph {S}_{ij}&= 
	V_i^2 (g_{ij} + g_{\mathrm{s}i}) - 
	\mathrm{j}V_i^2(b_{ij} + b_{\mathrm{s}i}) -
	V_iV_j\mathrm{e}^{\mathrm{j}\theta_{ij}}(g_{ij} - \mathrm{j}b_{ij}),
	\end{aligned}
   	\label{apparent_state}
	\end{equation}
where $\theta_{ij} = \theta_i - \theta_j$ is the bus voltage angle difference between bus voltage angles at buses $i$ and $j$. The apparent power $\ph S_{ij}$ consists of the active $P_{ij}$ and reactive $Q_{ij}$ power flow \eqref{apparent_ij}. Hence, the real and imaginary components of the complex expression \eqref{apparent_state} define the active and reactive power flow measurement functions $P_{ij} \triangleq h_{P_{ij}}(\cdot)$ and $Q_{ij} \triangleq h_{Q_{ij}}(\cdot)$. 

\begin{tcolorbox}[title=Active and Reactive Power Flow Measurement Functions]
Thus, measurements $\{M_{P_{ij}},$ $M_{Q_{ij}}\} \in \mathcal{M}$, $(i,j) \in \mathcal{E}$ are associated with measurement functions:
	\begin{subequations}
   	\begin{align}
    h_{P_{ij}}(\cdot)&=
    {V}_{i}^2(g_{ij}+g_{si})-{V}_{i}{V}_{j}(g_{ij}\cos\theta_{ij}
    +b_{ij}\sin\theta_{ij})
    \label{mf_activeF}\\
    h_{Q_{ij}}(\cdot)&=
    -{V}_{i}^2(b_{ij}+b_{si})-{V}_{i}{V}_{j}(g_{ij}\sin\theta_{ij}
    -b_{ij}\cos\theta_{ij}).
    \label{mf_reactiveF}
   	\end{align}
   	\label{mf_flow}%
	\end{subequations}
\vspace{-0.7\baselineskip}	
\end{tcolorbox}

Jacobian expressions corresponding to the measurement function $h_{P_{ij}}(\cdot)$ are defined:
	\begin{subequations}
   	\begin{align}
    \cfrac{\mathrm \partial{h_{P_{ij}}(\cdot)}}
    {\mathrm \partial \theta_{i}}&=
    {V}_{i}{V}_{j}(g_{ij}\sin\theta_{ij}-b_{ij}\cos\theta_{ij}) 			
    \label{jac_ele_PijTi}
    \\
    \cfrac{\mathrm \partial{{h_{P_{ij}}}(\cdot)}}
    {\mathrm \partial \theta_{j}}&=
    -{V}_{i}{V}_{j}(g_{ij}\sin\theta_{ij}-b_{ij}\cos\theta_{ij})
    \label{jac_ele_PijTj}
    \\
    \cfrac{\mathrm \partial{{h_{P_{ij}}}(\cdot)}}
   	{\mathrm \partial V_{i}}&=
    -{V}_{j}(g_{ij}\cos\theta_{ij}+b_{ij}\sin\theta_{ij})+
    2V_{i}(g_{ij}+g_{si}) 
    \label{jac_ele_PijVi}
    \\
    \cfrac{\mathrm \partial{h_{{P_{ij}}}(\cdot)}}{\mathrm \partial V_{j}}&=
    -{V}_{i}(g_{ij}\cos\theta_{ij}+b_{ij}\sin\theta_{ij}). 
    \label{jac_ele_PijVj}    
	\end{align}
   	\label{jac_ele_Pij}%
	\end{subequations}  	
Further, Jacobian expressions corresponding to the measurement function $h_{Q_{ij}}(\cdot)$ are:
\begin{subequations}
   	\begin{align}
    \cfrac{\mathrm \partial{h_{{Q_{ij}}}(\cdot)}}
    {\mathrm \partial \theta_{i}}&=
    -{V}_{i}{V}_{j}(g_{ij}\cos\theta_{ij}+b_{ij}\sin\theta_{ij})
    \label{jac_ele_QijTi}
    \\
    \cfrac{\mathrm \partial{h_{{Q_{ij}}}(\cdot)}}
    {\mathrm \partial \theta_{j}}&=
    {V}_{i}{V}_{j}(g_{ij}\cos\theta_{ij}+b_{ij}\sin\theta_{ij})
    \label{jac_ele_QijTj}
    \\
    \cfrac{\mathrm \partial{h_{{Q_{ij}}}(\cdot)}}{\mathrm \partial V_{i}}&=
    -{V}_{j}(g_{ij}\sin\theta_{ij}-b_{ij}\cos\theta_{ij})-
    2V_{i}(b_{ij}+b_{si})
	\label{jac_ele_QijVi}    
    \\
    \cfrac{\mathrm \partial{h_{{Q_{ij}}}(\cdot)}}
    {\mathrm \partial V_{j}}&=-
    {V}_{i}(g_{ij}\sin\theta_{ij}-b_{ij}\cos\theta_{ij}).
    \label{jac_ele_QijVj}
	\end{align}
   	\label{jac_ele_Qij}%
	\end{subequations}

The line current magnitude at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ can be obtained using \eqref{apparent_ij}:  
	\begin{equation}
   	\begin{aligned}
	I_{ij} = \cfrac{\sqrt{P_{ij}^2 + Q_{ij}^2}}{V_i}.
	\end{aligned}
   	\label{curmag_flow}
	\end{equation}
Using \eqref{mf_flow} and \eqref{curmag_flow}, the expression that defines the line current magnitude measurement function $I_{ij} \triangleq h_{I_{ij}}(\cdot)$ can be obtained.

\begin{tcolorbox}[title=Line Current Magnitude Measurement Function]	
Hence, measurement $M_{I_{ij}}$ $\in$ $\mathcal{M}$, $(i,j) \in \mathcal{E}$ is associated with measurement function:
	\begin{equation}
	h_{I_{ij}}(\cdot) = 
    [A_\mathrm{c} V_i^2 + B_\mathrm{c} V_j^2 - 2 V_iV_j
    (C_\mathrm{c} \cos \theta_{ij}-D_\mathrm{c} \sin \theta_{ij})]^{1/2},
    \label{mf_curmag}
	\end{equation}	
where coefficients are as follows: 		
	\begin{equation}
    \begin{aligned}
    A_\mathrm{c}&=(g_{ij}+g_{\mathrm{s}i})^2+(b_{ij}+b_{\mathrm{s}i})^2;&
    B_\mathrm{c}&=g_{ij}^2+b_{ij}^2\\
    C_\mathrm{c}&=g_{ij}(g_{ij}+g_{\mathrm{s}i})+b_{ij}(b_{ij}+b_{\mathrm{s}i});&
    D_\mathrm{c}&=g_{ij}b_{\mathrm{s}i}-b_{ij}g_{\mathrm{s}i}.
    \end{aligned}
    \nonumber
	\end{equation}
\end{tcolorbox}

Jacobian expressions corresponding to the line current magnitude measurement function $h_{I_{ij}}(\cdot)$ are:  
	\begin{subequations}
   	\begin{align}
	\cfrac{\mathrm \partial{h_{I_{ij}}(\cdot)}}
	{\mathrm \partial \theta_{i}}&=
    \cfrac{V_iV_j(D_\mathrm{c}\cos\theta_{ij}+
    C_\mathrm{c}\sin\theta_{ij})}{h_{I_{ij}}(\cdot)}
    \label{jac_ele_IijTi}	
    \\
    \cfrac{\mathrm \partial{h_{I_{ij}}(\cdot)}}
    {\mathrm \partial \theta_{j}}&=-
    \cfrac{V_iV_j(D_\mathrm{c}\cos\theta_{ij}+
    C_\mathrm{c}\sin\theta_{ij})}{h_{I_{ij}}(\cdot)}
    \label{jac_ele_IijTj}
    \\
    \cfrac{\mathrm \partial{h_{I_{ij}}(\cdot)}}{\mathrm \partial V_{i}}&=
    \cfrac{V_j(D_\mathrm{c}\sin\theta_{ij}-
    C_\mathrm{c}\cos\theta_{ij})+A_\mathrm{c}V_i}{h_{I_{ij}}(\cdot)}
    \label{jac_ele_IijVi}
    \\
    \cfrac{\mathrm \partial{h_{I_{ij}}(\cdot)}}{\mathrm \partial V_{j}}&=
    \cfrac{V_i(D_\mathrm{c}\sin\theta_{ij}-
    C_\mathrm{c}\cos\theta_{ij})+B_\mathrm{c}V_j}{h_{I_{ij}}(\cdot)}. 
    \label{jac_ele_IijVj}   
	\end{align}
   	\label{jac_ele_Iij}%
	\end{subequations}	

Note that, in deregulation environment current magnitude measurements can be found in significant numbers, especially in distribution grids. The use of line current magnitude measurements can lead to various problems (e.g., the ``flat start" will cause undefined Jacobian elements), which in turn may seriously deteriorate the performance of the state estimators \cite[Sec.~9.3]{abur}.

The active and reactive power injection into the bus $i \in \mathcal{H}$ can be obtained using \eqref{apparent_inj} and \eqref{apparent_inj_state}, where the real and imaginary components determine the active and reactive power injection measurement functions $P_{i} \triangleq h_{P_{i}}(\cdot)$ and $Q_{i} \triangleq h_{Q_{i}}(\cdot)$.

\begin{tcolorbox}[title=Active and Reactive Power Injection Measurement Functions]
Thus, measurements $\{M_{P_{i}},$ $M_{Q_{i}}\}$ $\in$ $\mathcal{M}$, $i \in \mathcal{H}$ are associated with measurement functions: 
	\begin{subequations}
   	\begin{align}
    h_{P_{i}}(\cdot) &={V}_{i}\sum\limits_{j \in \mathcal{H}_i} {V}_{j}
    (G_{ij}\cos\theta_{ij}+B_{ij}\sin\theta_{ij})\label{mf_injcetionA}\\
    h_{Q_{i}}(\cdot) &={V}_{i}\sum\limits_{j \in \mathcal{H}_i} {V}_{j}
    (G_{ij}\sin\theta_{ij}-B_{ij}\cos\theta_{ij})\label{mf_injcetionR}.     
	\end{align}
   	\label{mf_injcetion}%
	\end{subequations}
\vspace{-1.0\baselineskip}
\end{tcolorbox}
 
Jacobian expressions corresponding to the measurement function $h_{P_{i}}(\cdot)$ are defined:
	\begin{subequations}
   	\begin{align}
    \cfrac{\mathrm \partial{h_{P_{i}}(\cdot)}}
    {\mathrm \partial \theta_{i}}&=
    {V}_{i}\sum_{j \in \mathcal{H}_i \setminus i } {V}_{j}
    (-G_{ij}\sin\theta_{ij}+B_{ij}\cos\theta_{ij})
    \label{jac_ele_PiTi}
    \\
    \cfrac{\mathrm \partial{h_{P_{i}}(\cdot)}}{\mathrm \partial \theta_{j}}&=
    {V}_{i}{V}_{j}(G_{ij}\sin\theta_{ij}-B_{ij}\cos\theta_{ij})
    \label{jac_ele_PiTj}
    \\
    \cfrac{\mathrm \partial{h_{P_{i}}(\cdot)}}{\mathrm \partial V_{i}}&=
    \sum_{j \in \mathcal{H}_i \setminus i } 
    {V}_{j}(G_{ij}\cos\theta_{ij}+B_{ij}
    \sin\theta_{ij})+2{V}_{i}G_{ii}
    \label{jac_ele_PiVi}
    \\
    \cfrac{\mathrm \partial{h_{P_{i}}(\cdot)}}{\mathrm \partial V_{j}}&=
    {V}_{i}(G_{ij}\cos\theta_{ij}+B_{ij}\sin\theta_{ij}),
    \label{jac_ele_PiVj}
	\end{align}
   	\label{jac_ele_Pi}%
	\end{subequations}
where $\mathcal{H}_i \setminus i$ is the set of buses adjacent to the bus $i$. Furthermore, Jacobian expressions corresponding to the measurement function $h_{Q_{i}}(\cdot)$ are:
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{Q_{i}}(\cdot)}}
   	{\mathrm \partial \theta_{i}}&=
    {V}_{i}\sum_{j \in \mathcal{H}_i \setminus i }
    {V}_{j}(G_{ij}\cos\theta_{ij}+B_{ij}\sin\theta_{ij})
    \label{jac_ele_QiTi}
    \\
    \cfrac{\mathrm \partial{h_{Q_{i}}(\cdot)}}{\mathrm \partial \theta_{j}}&=
    {V}_{i}{V}_{j}(-G_{ij}\cos\theta_{ij}-B_{ij}
    \sin\theta_{ij})
    \label{jac_ele_QiTj}
    \\
    \cfrac{\mathrm \partial{h_{Q_{i}}(\cdot)}}{\mathrm \partial V_{i}}&=
    \sum_{j \in \mathcal{H}_i \setminus i }
    {V}_{j}(G_{ij}\mbox{sni}\theta_{ij}-B_{ij}
    \cos\theta_{ij})-2{V}_{i}B_{ii}	
    \label{jac_ele_QiVi}
    \\
    \cfrac{\mathrm \partial{h_{Q_{i}}(\cdot)}}{\mathrm \partial V_{j}}&=
    {V}_{i}(G_{ij}\sin\theta_{ij}-B_{ij}\cos\theta_{ij}).  
    \label{jac_ele_QiVj}  
	\end{align}
   	\label{jac_ele_Qi}%
	\end{subequations}

The bus voltage magnitude on the bus $i \in \mathcal{H}$ simply defines corresponding measurement function $V_{i} \triangleq h_{V_{i}}(\cdot)$. 

\begin{tcolorbox}[title=Bus Voltage Magnitude Measurement Function]
Hence, measurement $M_{V_{i}}$ $\in$ $\mathcal{M}$, $i \in \mathcal{H}$ is associated with measurement function:
		\begin{equation}
        \begin{aligned}
        h_{V_{i}}(\cdot) = V_i.
        \end{aligned}
        \label{mf_voltage_leg}
		\end{equation} 
\end{tcolorbox}		 

Jacobian expressions corresponding to the measurement function $h_{V_{i}}(\cdot)$ are defined:  
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{{h_{V_{i}}(\cdot)}}}
   	{\mathrm \partial \theta_{i}}=0;\;\;\;\;  
    \cfrac{\mathrm \partial{{h_{V_{i}}(\cdot)}}}
    {\mathrm \partial \theta_{j}}=0   	
    \label{jac_ele_ViTiTj} \\   	
   	\cfrac{\mathrm \partial{{h_{V_{i}}(\cdot)}}}
   	{\mathrm \partial V_{i}}=1; \;\;\;\;  
    \cfrac{\mathrm \partial{{h_{V_{i}}(\cdot)}}}{\mathrm 
    \partial V_{j}}=0.	
    \label{jac_ele_ViViVj}
	\end{align}
   	\label{jac_ele_Vi}%
	\end{subequations}	

\subsection{The Conventional SE Model}
The conventional SE model implies the state vector in polar coordinates $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, where the vector of measurement functions $\mathbf h (\mathbf x)$ and corresponding Jacobian elements of the matrix $\mathbf J (\mathbf x)$ are expressed in the same coordinate system. If we denote with $N_{\mathrm{le}}$ the number of legacy measurements, the vector of measurement values  $\mathbf z_{\mathrm{le}} \in \mathbb {R}^{N_{\mathrm{le}}}$, the vector of measurement functions $\mathbf h_{\mathrm{le}}(\mathbf x) \in \mathbb {R}^{N_{\mathrm{le}}}$ and corresponding Jacobian matrix $\mathbf {J}_\mathrm{{le}}(\mathbf x) \in \mathbb {R}^{N_{\mathrm{le}} \times n}$ are: 
	\begin{equation}
   	\begin{gathered}
   	\mathbf z_{\mathrm{le}} =
    \begin{bmatrix}    	 
	\mathbf z_{\mathrm{P_{ij}}}\\[3pt]
	\mathbf z_{\mathrm{Q_{ij}}}\\[3pt]
	\mathbf z_{\mathrm{I_{ij}}}\\[3pt]
	\mathbf z_{\mathrm{P_{i}}}\\[3pt]
	\mathbf z_{\mathrm{Q_{i}}}\\[3pt]
	\mathbf z_{\mathrm{V_{i}}}
	\end{bmatrix};		
	\;\;\;\;   	
   	\mathbf h_{\mathrm{le}} (\mathbf x) =
    \begin{bmatrix}    	 
	\mathbf h_{\mathrm{P_{ij}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{Q_{ij}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{I_{ij}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{P_{i}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{Q_{i}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{V_{i}}}(\mathbf x)
	\end{bmatrix};		
	\;\;\;\;
    \mathbf J_{\mathrm{le}}(\mathbf x)=
    \begin{bmatrix} 
    \mathbf {J}_\mathrm{{P_{ij}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{P_{ij}V}}(\mathbf x)    \\[3pt]
    \mathbf {J}_\mathrm{{Q_{ij}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{Q_{ij}V}}(\mathbf x)    \\[3pt]	
	\mathbf {J}_\mathrm{{I_{ij}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{I_{ij}V}}(\mathbf x)    \\[3pt]    
    \mathbf {J}_\mathrm{{P_{i}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{P_{i}V}}(\mathbf x)    \\[3pt]
    \mathbf {J}_\mathrm{{Q_{i}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{Q_{i}V}} (\mathbf x)   \\[3pt]
	\mathbf {J}_\mathrm{{V_{i}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{V_{i}V}}(\mathbf x) 	 
	\end{bmatrix}.
	\end{gathered}
   	\label{mv_leg}
	\end{equation}
Due to assumption of uncorrelated measurement errors (i.e., usual assumption for legacy measurements), the measurement error covariance matrix $\mathbf{R}_\mathrm{le} \in \mathbb {R}^{N_{\mathrm{le}} \times N_{\mathrm{le}}}$ has the diagonal structure:
	\begin{equation}
   	\begin{gathered}
	\mathbf R_{\mathrm{le}} = \mathrm{diag}	
    (
	\mathbf R_{\mathrm{P_{ij}}},
	\mathbf R_{\mathrm{Q_{ij}}},
	\mathbf R_{\mathrm{I_{ij}}},
	\mathbf R_{\mathrm{P_{i}}},
	\mathbf R_{\mathrm{Q_{i}}},
	\mathbf R_{\mathrm{V_{i}}}),	
    \end{gathered}
   	\label{mv_cova_mat}
	\end{equation}
and each covariance sub-matrix of $\mathbf R_{\mathrm{le}}$ is the diagonal matrix that contains measurement variances.

The solution of the described SE model can be found using Gauss-Newton method, where $\mathbf z \equiv \mathbf z_{\mathrm{le}}$, $\mathbf h (\mathbf x) \equiv \mathbf h_{\mathrm{le}} (\mathbf x)$, $\mathbf J(\mathbf x) \equiv \mathbf J_{\mathrm{le}}(\mathbf x)$ and $\mathbf R\equiv \mathbf R_{\mathrm{le}}$. In \autoref{app:A}, we provide a step-by-step illustrative example to describe the SE model where legacy measurements are involved. 

\section{Phasor Measurements with Polar State Vector} \label{sub:pmu_meas}
Integration of phasor measurements in the established model with legacy measurements can be done using different approaches. To recall, phasor measurements contain line current $\mathcal{M}_{\ph{I}_{ij}}$, $(i,j) \in \mathcal{E}$ and bus voltage $\mathcal{M}_{\ph{V}_{i}}$, $i \in \mathcal{H}$ phasors. More precisely, phasor measurement provided by PMU is formed by a magnitude, equal to the root mean square value of the signal, and phase angle \cite[Sec.~5.6]{phadkeBook}, where measurement errors are also related with magnitude and angle of the phasor. Thus, the PMU outputs phasor measurement in polar coordinates. In addition, PMU outputs can be observed in the rectangular coordinates with real and imaginary parts of the bus voltage and line current phasors, but in that case, the two measurements may be affected by correlated measurement errors. \cite[Sec.~7.3]{phadkeBook}. Note that throughout this section the vector of state variables is given in polar coordinates $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$.

\subsection{Measurements in Polar Coordinates} \label{sub:pmu_polar}
In the majority of PMUs, the voltage and current phasors in polar coordinate system are regarded as ``direct'' measurements (i.e., output from the PMU). This representation delivers the more accurate state estimates in comparison to the rectangular measurement representation, but it requires larger computing time \cite{manousakis}. This representation is called simultaneous SE formulation, where measurements provided by PMUs are handled in the same manner as legacy measurements \cite{catalina}. Measurement errors are uncorrelated, with measurement variances that correspond to each components of the phasor measurements (i.e., magnitude and angle). 

The bus voltage phasor on the bus $i \in \mathcal{H}$ in the polar coordinate system is described:
	\begin{equation}
   	\begin{aligned}
    \ph V_i = V_{i}\mathrm{e}^{\mathrm{j}\theta_{i}},
   	\end{aligned}
   	\label{state_vol1}
	\end{equation} 
and due the fact that the state vector is given in the polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, measurement functions are defined as $V_{i} \triangleq h_{V_{i}}(\cdot)$, $\theta_{i} \triangleq h_{\theta_{i}}(\cdot)$. 

\begin{tcolorbox}[title=Bus Voltage Phasor Measurement Functions]
Measurement $\mathcal{M}_{\ph{V}_{i}}= $ $\{M_{{V}_{i}},$ $M_{{\theta}_{i}}\}$ $\subseteq$ $\mathcal{M}$, $i \in \mathcal{H}$ is associated with measurement functions:
	\begin{subequations}
   	\begin{align}
	h_{{V}_{i}}(\cdot) = V_i\\
	h_{\theta_i}(\cdot) = \theta_i.
    \end{align}    
   	\label{vol_pha_meas_fun}
	\end{subequations} 
\vspace{-1.0\baselineskip}	
\end{tcolorbox}	
	
Jacobian expressions corresponding to the measurement function $h_{{V}_{i}}(\cdot)$ are defined:  
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{{h_{{V}_{i}}(\cdot)}}}
   	{\mathrm \partial \theta_{i}}=0;\;\;\;\;  
    \cfrac{\mathrm \partial{{h_{{V}_{i}}(\cdot)}}}
    {\mathrm \partial \theta_{j}}=0   	
    \label{jac_ele_ViTiTj_pmu} \\   	
   	\cfrac{\mathrm \partial{{h_{{V}_{i}}(\cdot)}}}
   	{\mathrm \partial V_{i}}=1; \;\;\;\;  
    \cfrac{\mathrm \partial{{h_{{V}_{i}}(\cdot)}}}{\mathrm 
    \partial V_{j}}=0,	
    \label{jac_ele_ViViVj_pmu}
	\end{align}
   	\label{jac_ele_Vi_pmu}%
	\end{subequations}	
while Jacobian expressions corresponding to the measurement function $h_{\theta_i}(\cdot)$ are:  
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{{h_{\theta_i}(\cdot)}}}
   	{\mathrm \partial \theta_{i}}=1;\;\;\;\;  
    \cfrac{\mathrm \partial{{h_{\theta_i}(\cdot)}}}
    {\mathrm \partial \theta_{j}}=0   	
    \label{jac_ele_TiTiTj_pmu} \\   	
   	\cfrac{\mathrm \partial{{h_{\theta_i}(\cdot)}}}
   	{\mathrm \partial V_{i}}=0; \;\;\;\;  
    \cfrac{\mathrm \partial{{h_{\theta_i}(\cdot)}}}{\mathrm 
    \partial V_{j}}=0.	
    \label{jac_ele_TiViVj_pmu}
	\end{align}
   	\label{jac_ele_Ti_pmu}%
	\end{subequations}

The line current phasor at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ in polar coordinates is defined as:
	\begin{equation}
   	\begin{aligned}
	\mathscr{I}_{ij}&=I_{ij}\mathrm{e}^{\mathrm{j}\phi_{ij}},
    \end{aligned}    
   	\label{curr_pha}
	\end{equation}
where $I_{ij}$ and $\phi_{ij}$ are magnitude and angle of the line current phasor, respectively. The line current phasor measurement directly measures magnitude and angle of the phasor. It is easy to obtain magnitude and angle equations of the line current phasor using \eqref{current_ij}, where the vector of state variables is given in the polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$. Thus, the line current phasor measurement $\mathcal{M}_{\ph{I}_{ij}}= $ $\{M_{{I}_{ij}},$ $M_{{\phi}_{ij}}\}$ $\subseteq$ $\mathcal{M}$, $(i,j) \in \mathcal{E}$ is associated with magnitude $I_{ij} \triangleq h_{I_{ij}}(\cdot)$ and angle $\phi_{ij} \triangleq h_{\phi_{ij}}(\cdot)$ measurement functions.   
	
\begin{tcolorbox}[title=Magnitude of Line Current Phasor Measurement Function]	
To recall, measurement $M_{{I}_{ij}}$ $\in$ $\mathcal{M},$ $(i,j) \in \mathcal{E}$ is associated with measurement function:
	\begin{equation}
	h_{{I}_{ij}}(\cdot) = 
    [A_\mathrm{c} V_i^2 + B_\mathrm{c} V_j^2 - 2 V_iV_j
    (C_\mathrm{c} \cos \theta_{ij}-D_\mathrm{c} \sin \theta_{ij})]^{1/2},
    \label{mf_curmag_pmu}
	\end{equation}	
where coefficients are as follows: 		
	\begin{equation}
    \begin{aligned}
    A_\mathrm{c}&=(g_{ij}+g_{\mathrm{s}i})^2+(b_{ij}+b_{\mathrm{s}i})^2;&
    B_\mathrm{c}&=g_{ij}^2+b_{ij}^2\\
    C_\mathrm{c}&=g_{ij}(g_{ij}+g_{\mathrm{s}i})+b_{ij}(b_{ij}+b_{\mathrm{s}i});&
    D_\mathrm{c}&=g_{ij}b_{\mathrm{s}i}-b_{ij}g_{\mathrm{s}i}.
    \end{aligned}
    \nonumber
	\end{equation}
\end{tcolorbox}	
	
Jacobian expressions corresponding to the measurement function $h_{I_{ij}}(\cdot)$ are given in \eqref{jac_ele_Iij}.	

\begin{tcolorbox}[title=Angle of Line Current Phasor Measurement Function]			
Furthermore, measurement $M_{{\phi}_{ij}}$ $\in$ $\mathcal{M},$ $(i,j) \in \mathcal{E}$ is associated with measurement function:
	\begin{equation}
	h_{{\phi}_{ij}}(\cdot) =\mathrm{arctan}\Bigg[ 
	\cfrac{(A_\mathrm{a} \sin\theta_i
    +B_\mathrm{a} \cos\theta_i)V_i 
    - (C_\mathrm{a} \sin\theta_j + D_\mathrm{a}\cos\theta_j)V_j}
   	{(A_\mathrm{a} \cos\theta_i
    -B_\mathrm{a} \sin\theta_i)V_i 
    - (C_\mathrm{a} \cos\theta_j - D_\mathrm{a} \sin\theta_j)V_j} \Bigg],    
    \label{mf_curang}
	\end{equation}
where coefficients are as follows: 		
	\begin{equation}
    \begin{aligned}
    A_\mathrm{a}&=g_{ij}+g_{\mathrm{s}i};&
    B_\mathrm{a}&=b_{ij}+b_{\mathrm{s}i}\\
    C_\mathrm{a}&=g_{ij};&
    D_\mathrm{a}&=b_{ij}.
    \end{aligned}
    \nonumber
	\end{equation}	
\end{tcolorbox}	
	
Jacobian expressions corresponding to the measurement function $h_{{\phi}_{ij}}(\cdot)$ are:	
	\begin{subequations}
   	\begin{align}
	\cfrac{\mathrm \partial{h_{{\phi}_{ij}}(\cdot)}}
	{\mathrm \partial \theta_{i}}&=
	\frac{A_\mathrm{c} V_i^2+ (D_\mathrm{c} \sin \theta_{ij}-C_\mathrm{c} 
	\cos\theta_{ij})V_iV_j}
   	{h_{{I}_{ij}}(\cdot)}\\
   	\cfrac{\mathrm \partial{h_{{\phi}_{ij}}(\cdot)}}
	{\mathrm \partial \theta_{j}}&=
	\frac{B_\mathrm{c} V_j^2+ (D_\mathrm{c}
   	\sin \theta_{ij}-C_\mathrm{c} \cos
   	\theta_{ij})V_iV_j}{h_{{I}_{ij}}(\cdot)}	\\
   	\cfrac{\mathrm \partial{h_{{\phi}_{ij}}(\cdot)}}
	{\mathrm \partial V_{i}}&=
   	-\frac{V_j (C_\mathrm{c} \sin\theta_{ij}+D_\mathrm{c} \cos\theta_{ij})}
   	{h_{{I}_{ij}}(\cdot)}\\
   	\cfrac{\mathrm \partial{h_{{\phi}_{ij}}(\cdot)}}
	{\mathrm \partial V_{j}}&=
	\frac{V_i (C_\mathrm{c} \sin\theta_{ij}+D_\mathrm{c} \cos\theta_{ij})}
   	{h_{{I}_{ij}}(\cdot)}.		
	\end{align}
   	\label{jac_ele_Iij_pmu}%
	\end{subequations}

To summarize, presented measurement model associated with line current phasor measurements is non-linear. However, if we denote with $N_{\mathrm{ph}}$ the number of phasor measurements, the vector of measurement values  $\mathbf z_{\mathrm{ph}} \in \mathbb {R}^{2N_{\mathrm{ph}}}$, the vector of measurement functions $\mathbf h_{\mathrm{ph}}(\mathbf x) \in \mathbb {R}^{2N_{\mathrm{ph}}}$ and corresponding Jacobian matrix $\mathbf {J}_\mathrm{{ph}}(\mathbf x) \in \mathbb {R}^{(2N_{\mathrm{ph}}) \times n}$ are: 
	\begin{equation}
   	\begin{gathered}
   	\mathbf z_{\mathrm{ph}} =
    \begin{bmatrix}    	 
	\mathbf z_{\mathrm{V_{i}}}\\[3pt]
	\mathbf z_{\mathrm{\uptheta_{i}}}\\[3pt]
	\mathbf z_{\mathrm{I_{ij}}}\\[3pt]
	\mathbf z_{\mathrm{\upphi_{ij}}}
	\end{bmatrix};		
	\;\;\;\;   	
   	\mathbf h_{\mathrm{ph}} (\mathbf x) =
    \begin{bmatrix}    	 
	\mathbf h_{\mathrm{V_{i}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{\uptheta_{i}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{I_{ij}}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{\upphi_{i}}}(\mathbf x)
	\end{bmatrix};		
	\;\;\;\;
    \mathbf J_{\mathrm{ph}}(\mathbf x)=
    \begin{bmatrix} 
    \mathbf {J}_\mathrm{{V_{i}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{V_{i}V}}(\mathbf x)    \\[3pt]
    \mathbf {J}_\mathrm{{\uptheta_{i}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{\uptheta_{i}V}}(\mathbf x)    \\[3pt]	
	\mathbf {J}_\mathrm{{I_{ij}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{I_{ij}V}}(\mathbf x)    \\[3pt]    
    \mathbf {J}_\mathrm{{\upphi_{ij}\uptheta}}(\mathbf x) &
	\mathbf {J}_\mathrm{{\upphi_{ij}V}}(\mathbf x)	 
	\end{bmatrix}.
	\end{gathered}
   	\label{mv_pmu_pol}
	\end{equation}

When phasor measurements are given in polar coordinate system, measurement errors are uncorrelated and assume zero-mean Gaussian distribution whose covariance matrix $\mathbf{R}_\mathrm{ph} \in \mathbb {R}^{(2N_{\mathrm{ph}}) \times (2N_{\mathrm{ph}})}$ has the diagonal structure:
	\begin{equation}
   	\begin{gathered}
	\mathbf R_{\mathrm{ph}} = \mathrm{diag}	
    (
	\mathbf R_{\mathrm{V_{i}}},
	\mathbf R_{\mathrm{\uptheta_{i}}},
	\mathbf R_{\mathrm{I_{ij}}},
	\mathbf R_{\mathrm{\upphi_{ij}}}),	
    \end{gathered}
   	\label{mv_cova_pmu_pol}
	\end{equation}
where each covariance sub-matrix of $\mathbf R_{\mathrm{ph}}$ is the diagonal matrix that contains measurement variances.

The solution of the SE model with legacy and phasor measurements can be found using Gauss-Newton method, where:
	\begin{equation}
   	\begin{gathered}
   	\mathbf z \equiv
    \begin{bmatrix}    	 
	\mathbf z_{\mathrm{le}}\\[3pt]
	\mathbf z_{\mathrm{ph}}
	\end{bmatrix};		
	\;\;\;\;   	
   	\mathbf h (\mathbf x) \equiv
    \begin{bmatrix}    	 
	\mathbf h_{\mathrm{le}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{ph}}(\mathbf x)
	\end{bmatrix};		
	\;\;\;\;
    \mathbf J(\mathbf x)\equiv
    \begin{bmatrix} 
    \mathbf J_{\mathrm{le}}(\mathbf x)\\[3pt]
    \mathbf J_{\mathrm{ph}}(\mathbf x)
	\end{bmatrix}\;\;\;\;
	\mathbf R \equiv
    \begin{bmatrix}    	 
	\mathbf R_{\mathrm{le}} & \mathbf{0}\\
	\mathbf{0} &\mathbf R_{\mathrm{ph}}
	\end{bmatrix}.		
	\end{gathered}
   	\label{mv_pmu_pol_all}
	\end{equation}
In \autoref{app:A}, we provide a step-by-step illustrative example to describe the SE model with legacy and phasor measurements. 

\subsection{Measurements in Rectangular Coordinates} \label{sub:pmu_rect}
The bus voltage and line current phasors in rectangular coordinate system are regarded as ``indirect'' measurements obtained from measurements in polar coordinates \cite{manousakis}. Thus, measurements contain the real and imaginary parts of the line current phasor measurement and the real and imaginary parts of the bus voltage phasor measurement. As before, the vector of state variables is given in polar coordinates $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$.

The bus voltage phasor on the bus $i \in \mathcal{H}$ in the rectangular coordinate system is given: 
	\begin{equation}
   	\begin{aligned}
	\ph{V}_{i}&=\Re(\ph{V}_{i}) +\mathrm{j}\Im(\ph{V}_{i}). 
    \end{aligned}    
   	\label{vol_pha_rct}
	\end{equation}
The state vector is given in polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, hence using \eqref{vol_polar1}, one can obtain the real and imaginary components that define corresponding measurement functions $\Re(\ph{V}_{i}) \triangleq h_{\Re (\ph{V}_{i})}(\cdot)$ and $\Im(\ph{V}_{i}) \triangleq h_{\Im (\ph{V}_{i})}(\cdot)$, respectively.
	
\begin{tcolorbox}[title=Bus Voltage Phasor Measurement Functions]	
Measurement $\mathcal{M}_{\ph{V}_{i}}= $ $\{M_{{\Re (\ph{V}_{i})}},$ $M_{{\Im (\ph{V}_{i})}}\}$ $\subseteq$ $\mathcal{M}$, $i \in \mathcal{H}$ is associated with measurement functions:
	\begin{subequations}
   	\begin{align}
    h_{\Re (\ph{V}_{i})}(\cdot) &= V_i \cos\theta_i
    \label{mf_voltage_pmuRe}\\
    h_{\Im (\ph{V}_{i})}(\cdot) &= V_i \sin\theta_i. 
    \label{mf_voltage_pmuIm}   
	\end{align}
   	\label{mf_voltage_pmu_rct}%
	\end{subequations}	
\vspace{-1.5\baselineskip}		
\end{tcolorbox}

Jacobians expressions corresponding to the measurement function $h_{\Re (\ph{V}_{i})}(\cdot)$ are defined:
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \theta_{i}}=
    -V_i \sin\theta_i;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \theta_{j}}=0 \\
   	\cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial V_{i}}=
    \cos\theta_i;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial V_{j}}=0,    
	\end{align}
   	\label{jac_ele_pmuRe_Vi}%
	\end{subequations}
while Jacobians expressions corresponding to the measurement function $h_{\Im (\ph{V}_{i})}(\cdot)$ are: 
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \theta_{i}}=
    V_i \cos\theta_i;\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \theta_{j}}=0\\
    \cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial V_{i}}=
    \sin\theta_i;\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial V_{j}}=0.
	\end{align}
   	\label{jac_ele_pmuIm_Vi}%
	\end{subequations}	

In contrast to measurements represented in the polar coordinates, measurement functions and corresponding Jacobian elements are non-linear functions, which makes the polar coordinate system preferable.  

The line current phasor at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ in the rectangular coordinate system is given: 
	\begin{equation}
   	\begin{aligned}
	\ph{I}_{ij}&=\Re(\ph{I}_{ij}) +\mathrm{j}\Im(\ph{I}_{ij}). 
    \end{aligned}    
   	\label{vol_pha_rct1}
	\end{equation}
Using \eqref{current_ij} and \eqref{vol_polar}, where the state vector is given in polar coordinate system $\mathbf x \equiv[\bm \uptheta,\mathbf V]^{\mathrm{T}}$, the real and imaginary components of the line current phasor $\ph{I}_{ij}$ define measurement functions $\Re (\ph{I}_{ij}) \triangleq h_{\Re (\ph{I}_{ij})}(\cdot)$ and $\Im (\ph{I}_{ij}) \triangleq h_{\Im (\ph{I}_{ij})}(\cdot)$. 
	
\begin{tcolorbox}[title=Line Current Phasor Measurement Functions]	
Consequently, measurement $M_{\ph{I}_{ij}} = $ $\{M_{{\Re (\ph{I}_{ij})}},$ $M_{{\Im (\ph{I}_{ij})}}\}$ $\subseteq$ $\mathcal{M}$, $(i,j) \in \mathcal{E}$ is associated with measurement functions: 
	\begin{subequations}
   	\begin{align}
    h_{\Re (\ph{I}_{ij})}(\cdot) &= 
    V_i(A_\mathrm{a} \cos\theta_i - 
    B_\mathrm{a}\sin\theta_i) - 
    V_j(C_\mathrm{a}\cos\theta_j - 
    D_\mathrm{a}\sin\theta_j)\label{mf_current_pmuRe}\\
    h_{\Im (\ph{I}_{ij})}(\cdot) &=
    V_i(A_\mathrm{a}\sin\theta_i + 
    B_\mathrm{a}\cos\theta_i) - 
    V_j(C_\mathrm{a}\sin\theta_j + D_\mathrm{a}\cos\theta_j)\label{mf_current_pmuIm}.     
	\end{align}
   	\label{mf_current_pmu}%
	\end{subequations}
\vspace{-1.0\baselineskip}		
\end{tcolorbox}

Jacobians expressions corresponding to the measurement function $h_{\Re (\ph{I}_{ij})}(\cdot)$ are defined:	
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \theta_{i}}&=
    -V_i (A_\mathrm{a} \sin\theta_i + B_\mathrm{a}\cos\theta_i)\\
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \theta_{j}}&=
    V_j (C_\mathrm{a} \sin\theta_j + D_\mathrm{a}\cos\theta_j)
    \\
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial V_{i}}&=
    A_\mathrm{a} \cos\theta_i - B_\mathrm{a}\sin\theta_i\\
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial V_{j}}&=
    -C_\mathrm{a} \cos\theta_j + D_\mathrm{a}\sin\theta_j,
	\end{align}
   	\label{jac_ele_pmuRe_Iij}%
	\end{subequations}
while Jacobians expressions corresponding to the measurement function $h_{\Im (\ph{I}_{ij})}(\cdot)$ are:
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \theta_{i}}&=
    V_i (A_\mathrm{a} \cos\theta_i - B_\mathrm{a}\sin\theta_i)\\
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \theta_{j}}&=
    -V_j (C_\mathrm{a} \cos\theta_j - D_\mathrm{a}\sin\theta_j)
    \\
   	\cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial V_{i}}&=
    A_\mathrm{a} \sin\theta_i + B_\mathrm{a}\cos\theta_i\\
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial V_{j}}&=
    -C_\mathrm{a} \sin\theta_j - D_\mathrm{a}\cos\theta_j.    
	\end{align}
   	\label{jac_ele_pmuIm_Iij}%
	\end{subequations}

Same as before, functions associated with line current phasor measurements are non-linear. In addition, the rectangular representation of the line current phasor resolves ill-conditioned problems that arise in polar coordinates due to small values of current magnitudes \cite{manousakis, catalina}. The main disadvantage of this approach is related to measurement errors, because measurment errors correspond to polar coordinates (i.e. magnitude and phase errors), and hence, the covariance matrix must be transformed from polar to rectangular coordinates \cite{poor_wu, phadke, nuquistate}. As a result, measurement errors of a single PMU are correlated and covariance matrix does not have diagonal form. Despite that, the measurement error covariance matrix is usually considered as diagonal matrix, which has the effect on the accuracy of the SE. Note that, combining representation of measurements in polar and rectangular is possible, for example, the bus voltage phasor in polar form and the line current phasor in rectangular form is often used \cite{catalina}. 

The vector of measurement values  $\mathbf z_{\mathrm{ph}} \in \mathbb {R}^{2N_{\mathrm{ph}}}$, the vector of measurement functions $\mathbf h_{\mathrm{ph}}(\mathbf x) \in \mathbb {R}^{2N_{\mathrm{ph}}}$ and corresponding Jacobian matrix $\mathbf {J}_\mathrm{{ph}}(\mathbf x) \in \mathbb {R}^{(2N_{\mathrm{ph}}) \times n}$ are: 
	\begin{equation}
   	\begin{gathered}
   	\mathbf z_{\mathrm{ph}} =
    \begin{bmatrix}    	 
	\mathbf z_{\Re (\mathrm{\ph{V}_{i}})}\\[3pt]
	\mathbf z_{\Im (\mathrm{\ph{V}_{i}})}\\[3pt]
	\mathbf z_{\Re (\mathrm{\ph{I}_{ij}})}\\[3pt]
	\mathbf z_{\Im (\mathrm{\ph{I}_{ij}})}	
	\end{bmatrix};		
	\;\;\;   	
   	\mathbf h_{\mathrm{ph}} (\mathbf x) =
    \begin{bmatrix} 
	\mathbf h_{\Re (\mathrm{\ph{V}_{i}})}(\mathbf x)\\[3pt]
	\mathbf h_{\Im (\mathrm{\ph{V}_{i}})}(\mathbf x)\\[3pt]
	\mathbf h_{\Re (\mathrm{\ph{I}_{ij}})}(\mathbf x)\\[3pt]
	\mathbf h_{\Im (\mathrm{\ph{I}_{ij}})}(\mathbf x)	       	 
	\end{bmatrix}		
	\\
    \mathbf J_{\mathrm{ph}}(\mathbf x)=
    \begin{bmatrix}  
	\mathbf {J}_{\Re (\mathrm{\ph{V}_{i}})\uptheta}(\mathbf x) &
	\mathbf {J}_{\Re (\mathrm{{\ph{V}_{i}})V}}(\mathbf x) \\[3pt]
	\mathbf {J}_{\Im (\mathrm{\ph{V}_{i}})\uptheta}(\mathbf x) &
	\mathbf {J}_{\Im (\mathrm{{\ph{V}_{i}})V}} (\mathbf x) \\[3pt]
	\mathbf {J}_{\Re (\mathrm{\ph{I}_{ij}})\uptheta}(\mathbf x) &
	\mathbf {J}_{\Re (\mathrm{{\ph{I}_{ij}})V}}(\mathbf x) \\[3pt]
	\mathbf {J}_{\Im (\mathrm{\ph{I}_{ij}})\uptheta}(\mathbf x) &
	\mathbf {J}_{\Im (\mathrm{{\ph{I}_{ij}})V}}(\mathbf x)	
	\end{bmatrix}.
    \end{gathered}
   	\label{mv_pmu1}
	\end{equation}

In case we neglect correlation between the measurements of a single PMU, the matrix $\mathbf{R}_\mathrm{ph} \in \mathbb {R}^{(2N_{\mathrm{ph}}) \times (2N_{\mathrm{ph}})}$ can be observed as the diagonal matrix:
	\begin{equation}
   	\begin{gathered}
	\mathbf R_{\mathrm{ph}} = \mathrm{diag}(	
	\mathbf R_{\Re (\mathrm{\ph{V}_{i}})},
	\mathbf R_{\Im (\mathrm{\ph{V}_{i}})},
	\mathbf R_{\Re (\mathrm{\ph{I}_{ij}})},
	\mathbf R_{\Im (\mathrm{\ph{I}_{ij}})}),	 
    \end{gathered}
   	\label{mv_pmu2}
	\end{equation}
where each covariance sub-matrix of $\mathbf R_{\mathrm{ph}}$ is the diagonal matrix that contains measurement variances. To recall, the solution of the SE model with legacy and phasor measurements can be found using the Gauss-Newton method, where:
	\begin{equation}
   	\begin{gathered}
   	\mathbf z \equiv
    \begin{bmatrix}    	 
	\mathbf z_{\mathrm{le}}\\[3pt]
	\mathbf z_{\mathrm{ph}}
	\end{bmatrix};		
	\;\;\;\;   	
   	\mathbf h (\mathbf x) \equiv
    \begin{bmatrix}    	 
	\mathbf h_{\mathrm{le}}(\mathbf x)\\[3pt]
	\mathbf h_{\mathrm{ph}}(\mathbf x)
	\end{bmatrix};		
	\;\;\;\;
    \mathbf J(\mathbf x)\equiv
    \begin{bmatrix} 
    \mathbf J_{\mathrm{le}}(\mathbf x)\\[3pt]
    \mathbf J_{\mathrm{ph}}(\mathbf x)
	\end{bmatrix}\;\;\;\;
	\mathbf R \equiv
    \begin{bmatrix}    	 
	\mathbf R_{\mathrm{le}} & \mathbf{0}\\
	\mathbf{0}&\mathbf R_{\mathrm{ph}}
	\end{bmatrix}.		
	\end{gathered}
   	\label{mv_pmu_pol_all1}
	\end{equation}


\section{Phasor Measurements with Rectangular State Vector} \label{sub:pmu_linear}
For the case when the vector of state variables is given in rectangular coordinates $\mathbf x \equiv[\mathbf{V}_\mathrm{re},\mathbf{V}_\mathrm{im}]^{\mathrm{T}}$, and where measurements are also represented in the same coordinates, we obtain linear measurement functions with constant Jacobian elements. Unfortunately, direct inclusion in the conventional SE model is not possible due to different coordinate systems, however, this still represents the important advantage of phasor measurements. 

The bus voltage phasor on the bus $i \in \mathcal{H}$ in the rectangular coordinates is defined as:
	\begin{equation}
   	\begin{aligned}
	\ph{V}_{i}&=\Re(\ph{V}_{i}) +\mathrm{j}\Im(\ph{V}_{i}). 
    \end{aligned}    
   	\label{vol_pha_rct_rc}
	\end{equation}
The state vector is given in the rectangular coordinate system $\mathbf x \equiv[\mathbf{V}_\mathrm{re},\mathbf{V}_\mathrm{im}]^{\mathrm{T}}$ and the real and imaginary components of \eqref{vol_pha_rct_rc} directly define measurement functions $\Re(\ph{V}_{i}) \triangleq h_{\Re (\ph{V}_{i})}(\cdot)$ and $\Im(\ph{V}_{i}) \triangleq h_{\Im (\ph{V}_{i})}(\cdot)$.

\begin{tcolorbox}[title=Bus Voltage Phasor Measurement Functions]	
Measurement $\mathcal{M}_{\ph{V}_{i}}= $ $\{M_{{\Re (\ph{V}_{i})}},$ $M_{{\Im (\ph{V}_{i})}}\}$ $\subseteq$ $\mathcal{M}$, $i \in \mathcal{H}$ is associated with measurement functions:
	\begin{subequations}
   	\begin{align}
    h_{\Re (\ph{V}_{i})}(\cdot) &= \Re(\ph{V}_{i})
    \label{mf_voltage_pmuRe_rc}\\
    h_{\Im (\ph{V}_{i})}(\cdot) &= \Im(\ph{V}_{i}). 
    \label{mf_voltage_pmuIm_rc}   
	\end{align}
   	\label{mf_voltage_pmu_rct_rc}%
	\end{subequations}	
\vspace{-1.0\baselineskip}		
\end{tcolorbox}

Jacobians expressions corresponding to the measurement function $h_{\Re (\ph{V}_{i})}(\cdot)$ are defined:
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \Re(\ph{V}_{i})}=1;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \Re(\ph{V}_{j})}=0 \\
   	\cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \Im(\ph{V}_{i})}=0;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Re (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \Im(\ph{V}_{j})}=0,    
	\end{align}%
	\end{subequations}
while Jacobians expressions corresponding to the measurement function $h_{\Im (\ph{V}_{i})}(\cdot)$ are: 
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \Re(\ph{V}_{i})}=0;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \Re(\ph{V}_{j})}=0 \\
   	\cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
   	{\mathrm \partial \Im(\ph{V}_{i})}=1;\;\;\;\;  
    \cfrac{\mathrm \partial{h_{\Im (\ph{V}_{i})}(\cdot)}}
    {\mathrm \partial \Im(\ph{V}_{j})}=0.    
	\end{align}%
	\end{subequations}	

The line current phasor at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ in the rectangular coordinate system is given: 
	\begin{equation}
   	\begin{aligned}
	\ph{I}_{ij}&=\Re(\ph{I}_{ij}) +\mathrm{j}\Im(\ph{I}_{ij}). 
    \end{aligned}    
   	\label{vol_pha_rct2}
	\end{equation}
Using \eqref{current_ij} and \eqref{vol_polar}, where the state vector is given in the rectangular coordinate system $\mathbf x \equiv[\mathbf{V}_\mathrm{re},\mathbf{V}_\mathrm{im}]^{\mathrm{T}}$, the real and imaginary components of the line current phasor $\ph{I}_{ij}$ define measurement functions $\Re (\ph{I}_{ij}) \triangleq h_{\Re (\ph{I}_{ij})}(\cdot)$ and $\Im (\ph{I}_{ij}) \triangleq h_{\Im (\ph{I}_{ij})}(\cdot)$. 

\begin{tcolorbox}[title=Line Current Phasor Measurement Functions]	
Measurements $M_{\ph{I}_{ij}} = $ $\{M_{{\Re (\ph{I}_{ij})}},$ $M_{{\Im (\ph{I}_{ij})}}\}$ $\subseteq$ $\mathcal{M}$, $(i,j) \in \mathcal{E}$ are associated with measurement functions: 
	\begin{subequations}
   	\begin{align}
	h_{\Re (\ph{I}_{ij})}(\cdot) & = (g_{ij}+g_{\mathrm{s}i})\Re(\ph{V}_{i}) -
	(b_{ij}+b_{\mathrm{s}i})\Im(\ph{V}_{i}) - g_{ij}\Re(\ph{V}_{j}) +
	b_{ij}\Im(\ph{V}_{j})  
	\\
	h_{\Im (\ph{I}_{ij})}(\cdot) & = (b_{ij}+b_{\mathrm{s}i})\Re(\ph{V}_{i}) +
	(g_{ij}+g_{\mathrm{s}i})\Im(\ph{V}_{i}) - b_{ij}\Re(\ph{V}_{j}) -
	g_{ij}\Im(\ph{V}_{j}).  
	\end{align}%
	\end{subequations}	
\vspace{-1.0\baselineskip}		
\end{tcolorbox}

Jacobians expressions corresponding to the measurement function $h_{\Re (\ph{I}_{ij})}(\cdot)$ are defined:	
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \Re(\ph{V}_{i})}=
    g_{ij}+g_{\mathrm{s}i};\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \Re(\ph{V}_{j})}=
    -g_{ij}
    \\
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \Im(\ph{V}_{i})}=
    -b_{ij}-b_{\mathrm{s}i};\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Re (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \Im(\ph{V}_{j})}=
    b_{ij},
	\end{align}%
	\end{subequations}
while Jacobians expressions corresponding to the measurement function $h_{\Im (\ph{I}_{ij})}(\cdot)$ are: 
	\begin{subequations}
   	\begin{align}
   	\cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \Re(\ph{V}_{i})}=
    b_{ij}+b_{\mathrm{s}i};\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \Re(\ph{V}_{j})}=
    -b_{ij}
    \\
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
   	{\mathrm \partial \Im(\ph{V}_{i})}=
    g_{ij}+g_{\mathrm{s}i};\;\;\;\; 
    \cfrac{\mathrm \partial{h_{\Im (\ph{I}_{ij})}(\cdot)}}
    {\mathrm \partial \Im(\ph{V}_{j})}=
    -g_{ij}.
	\end{align}%
	\end{subequations}

To summarize, presented model represents system of linear equations, where solution can be found by solving the linear WLS problem. As before, measurement errors by a single PMU are correlated and covariance matrix does not hold diagonal form. 
	
\section{The DC State Estimation} \label{sec:dc_se_model}
The DC model is obtained by linearisation of the non-linear model. In the typical operating conditions, the difference of bus voltage angles between adjacent buses $(i,j) \in \mathcal{E}$ is very small $\theta_{i}-\theta_{j} \approx 0$, which implies $\cos \theta_{ij}\approx1$ and $\sin \theta_{ij} \approx \theta_{ij}$. Further, all bus voltage magnitudes are $V_i \approx 1$, $i \in \mathcal{H}$, and all shunt elements and branch resistances can be neglected. This implies that the DC model ignores the reactive powers and transmission losses and takes into account only the active powers. Therefore, the DC SE takes only bus voltage angles $\mathbf x \equiv {\bm \uptheta}^{\mathrm{T}}$ as state variables. Consequently, the number of state variables is $n=N-1$, where one voltage angle represents the slack bus\footnote{Similar to the non-linear SE, the BP approach uses complete set of state variables.}. 

The set of DC model measurements $\mathcal{M}$ involves only active power flow $M_{P_{ij}}$, $(i,j) \in \mathcal{E}$, and active power injection $M_{P_{i}}$, $i \in \mathcal{H}$, from legacy measurments, and without loss of generality, we can include bus voltage angle $M_{\theta_{i}}$, $i \in \mathcal{H}$, from PMUs. 

\begin{tcolorbox}[title=Linear Weighted Least-Squares Method]
The DC state estimate $\hat{\mathbf x} \equiv \hat{\bm \uptheta}{}^{\mathrm{T}}$, which is a solution to the WLS problem \eqref{SE_WLS_problem}, is obtained through the non-iterative procedure by solving the system of linear equations:  
		\begin{equation}
        \begin{aligned}  
		\Big(\mathbf H^\mathrm{T} {\mathbf R}^{-1} \mathbf H \Big) 
		\hat{\mathbf x} =		
		\mathbf H^\mathrm{T} {\mathbf R}^{-1} \mathbf z, \label{DC_WLS}\\
		\end{aligned}
        \end{equation}
where $\mathbf{H}\in \mathbb {R}^{k\mathrm{x}N}$ is the Jacobian matrix of measurement functions.
\end{tcolorbox}

According to the set of measurements $\mathcal{M}$, vector and matrices are the following block structure:
	\begin{equation}
   	\begin{gathered}
   	\mathbf z =
    \begin{bmatrix}    	 
	\mathbf z_{\mathrm{P_{ij}}}\\[3pt]
	\mathbf z_{\mathrm{P_{i}}}\\[3pt]
	\mathbf z_{\uptheta_{i}}
	\end{bmatrix};		
	\;\;\;\;   	
   	\mathbf {H} =
    \begin{bmatrix} 
    \mathbf {H}_\mathrm{{P_{ij}}}\\[3pt]
    \mathbf {H}_\mathrm{{P_{i}}}\\[3pt]
	\mathbf {H}_\mathrm{{\uptheta_{i}}}
	\end{bmatrix};	
	\;\;\;\;
	\mathbf R = 	
    \begin{bmatrix} 
	\mathbf R_{\mathrm{P_{ij}}}  & \mathbf{0}& \mathbf{0} \\
	\mathbf{0} & \mathbf R_{\mathrm{P_{i}}} & \mathbf{0}  \\
	\mathbf{0} &\mathbf{0} & \mathbf {R}_\mathrm{{\uptheta_{i}}}
	\end{bmatrix}.	
    \end{gathered}
   	\label{dc_mv_leg}
	\end{equation}
Note that, each sub-matrix of $\mathbf R$ is the diagonal measurement error covariance matrix that contains measurement variances. In the following, we provide expressions for elements of $\mathbf {H}$. 

\begin{tcolorbox}[title=Active Power Flow Measurement Function (DC Model)]
The active power flow at the branch $(i,j) \in \mathcal{E}$ that connects buses $i$ and $j$ can be obtained using \eqref{mf_activeF}:
	\begin{equation}
    \begin{aligned}
    h_{P_{ij}}(\cdot) &= 
    -b_{ij}(\theta_{i}-\theta_{j}).
    \end{aligned}
    \label{DC_active_flow}
    \end{equation}
\end{tcolorbox}
    
Jacobian $\mathbf {H}_\mathrm{{P_{ij}}}$ of the function $h_{P_{ij}}(\cdot)$ associated with measurement $M_{P_{ij}}$, $(i,j) \in \mathcal{E}$ is defined as matrix with corresponding elements:
	\begin{equation}
    \begin{aligned}
    \cfrac{\mathrm \partial{h_{P_{ij}}(\cdot)}}{\mathrm 
    \partial \theta_{i}}&=
    -b_{ij};\;\;\;\;
    \cfrac{\mathrm \partial{{h_{P_{ij}}}(\cdot)}}{\mathrm 
    \partial \theta_{j}}&=
    b_{ij}.
    \end{aligned}
    \label{DC_jac_Pij}%
    \end{equation}

\begin{tcolorbox}[title=Active Power Injection Measurement Function (DC Model)]
The active power injection into bus $i \in \mathcal{H}$ can be obtained using \eqref{mf_injcetionA}:
	\begin{equation}
    \begin{aligned}
    h_{P_{i}}(\cdot) &=
    -\sum_{j \in \mathcal{H}_i \setminus i} b_{ij}(\theta_{i}-\theta_{j}),
    \end{aligned}
    \label{DC_active_injection}
    \end{equation}
where $\mathcal{H}_i\setminus i$ is the set of buses adjacent to the bus $i$. 
\end{tcolorbox}

Jacobian $\mathbf {H}_\mathrm{{P_{i}}}$ of the function $h_{P_{i}}(\cdot)$ associated with measurement $M_{P_{i}}$, $i \in \mathcal{H}$ is defined as matrix with corresponding elements:		
	\begin{equation}
    \begin{aligned}
    \cfrac{\mathrm \partial{h_{P_{i}}(\cdot)}}
    {\mathrm \partial \theta_{i}}=
    -\sum_{j \in \mathcal{H}_i \setminus i} 
    b_{ij};\;\;\;\;
    \cfrac{\mathrm \partial{{h_{P_{i}}}(\cdot)}}
    {\mathrm \partial \theta_{j}}=
    \sum_{j \in \mathcal{H}_i \setminus i} b_{ij}.
    \end{aligned}
    \label{DC_jac_Pi}%
    \end{equation}

\begin{tcolorbox}[title=Bus Voltage Angle Measurement Function (DC Model)]
The bus voltage angle on the bus $i \in \mathcal{H}$ is described with function:
	\begin{equation}
    \begin{aligned}
    h_{\theta_{i}}(\cdot) = \theta_i. 
    \end{aligned}
    \label{DC_angle}
	\end{equation} 
\end{tcolorbox}

Jacobian $\mathbf {H}_\mathrm{{\uptheta_{i}}}$ of the function $h_{\theta_{i}}(\cdot)$ associated with measurement $M_{\theta_{i}}$, $i \in \mathcal{H}$ is defined as matrix with corresponding elements:
	\begin{equation}
    \begin{aligned}
	\cfrac{\mathrm \partial{{h_{\theta_{i}}(\cdot)}}}
	{\mathrm \partial \theta_{i}}=1;\;\;\;\;
	\cfrac{\mathrm \partial{{h_{\theta_{i}}(\cdot)}}}
	{\mathrm \partial \theta_{j}}=0.
    \end{aligned}
    \label{DC_jac_Ti}%
	\end{equation}


\section{Summary}
The solution for the non-linear and DC SE model can be found by solving the optimization problem \eqref{SE_likelihood}. The solution of the non-linear SE model reduces to solving the iterative Gauss-Newton method, while the DC SE solution can be obtained through the non-iterative procedure by solving WLS problem. The DC SE provides an approximate solution, where all bus voltage magnitudes are set to one. The presented models assume uncorrelated measurement errors that define diagonal measurement error covariance matrices.

In the SE problem, each measurement function $h_i(\mathbf x)$ depends on a limited (typically small) subset of state variables $\mathbf{x}$. Hence, the likelihood function $\mathcal{L}(\mathbf{z}|\mathbf{x})$ can be factorized into factors \eqref{SE_likelihood} affecting small subsets of state variables. \textit{This fact motivates solving the SE problem scalably and efficiently using probabilistic graphical models}. The solution involves defining the factor graph corresponding to \eqref{SE_likelihood}, and deriving expressions for BP messages exchanged over the factor graph.






==> first_pages/abstractsr.tex <==
\chap{Sa\v{z}etak} 
\pagestyle{empty}


TODO
Kada se u potpunosti definise sazetan na engleskom. Vidi da li je uopste potrebno da postoji kao dio disertacije, jer svakako ide prevod na srpski u onoj tabeli...
Kvacice:
mo\v{z}e
po\v{c}etku
re\v{s}enje
rezultuju\'{c}i



==> first_pages/acknowledgment.tex <==
\chap{Acknowledgments} 
\pagestyle{empty}


This thesis is a final result of an incredible journey that has lasted for the last four years. It is impossible to list all the incredible people that I met during this period, who left an indelible mark in my life. I would like to point out that the value of this thesis is not in mathematical equations, its main value is that it made me a better person. 

First and foremost, I would like to dedicate this thesis to my family, they have always been with me. I want to express my deep gratitude for their support, encouraging and love. 

Further, I would like to express my deepest gratitude to my friend and advisor Prof. Dejan Vukobratovic, without his support, nothing would be possible. There are simply no words to describe his influence on this work and on my life. You can meet such a person and scientist once in your life if you have the very best of luck, few people had so much positive influence on my life as he had. 

I owe very much to Dragana Bajovic, Dusan Jakovetic and Gorana Mijatovic, they were always there for me, without them these four years would be significantly different. Also, I would like to thank all members of the Communications and Signal Processing Group at Faculty of Technical Sciences, University of Novi Sad, 

I would like to give special thanks to ADVANTAGE and SENSIBLE projects, and special thanks to Hazel Cox, Prof. John Thompson, Prof. Cedomir Stefanovic, Charalampos Kalalas, Marko Angjelichinoski, Achilleas Tsitsimelis and Alexandros Kleidaras, for all wonderful moments that we shared through ADVANTAGE project. 

Finally, I owe my thanks to the great people who hosted me during my secondment time, Prof. Carles Anton-Haro, CTTC, Barcelona; Prof. Vladimir Stankovic, University of Strathclyde, Glasgow; Prof. Juraj Machaj, University of Zilina, Zilina; and Prof. Chao Wang, Tongji University, Shanghai.
 


==> first_pages/nomenclature_reset.tex <==
\thispagestyle{empty}

\vspace*{1cm}


\emph{The following chapters introduce new nomenclature.}


==> first_pages/quote.tex <==
\thispagestyle{empty}

\vspace*{1cm}

{\flushright \emph{Engineering: where the semi-skilled laborers \\execute the vision of those who think and dream. \\ Hello, Oompa Loompas of science.}\\Dr. Sheldon Lee Cooper, B.S., M.S., M.A., Ph.D., Sc.D.\\}





==> first_pages/title.tex <==
\thispagestyle{empty}


\begin{adjustwidth*}{-7.5mm}{-7.5mm}
\begin{flushleft}
{\LARGE \textsc{\textbf{Application of Deep Learning Methods \\ in Monitoring and Optimization \\ \vskip 2.1mm of Electric Power Systems}}}\\ \vskip 16mm
{\large \textbf{Ognjen Kunda\v{c}ina}}
\end{flushleft}
\end{adjustwidth*}

\pagebreak
\thispagestyle{empty}
\vspace*{9cm}

%\vskip 1cm
%Printed by SP Print, Novi Sad.\\
%\vskip 0.3cm
%\noindent ISBN 90--393--3663--6
% ISBN isbn number



